A Closer Look at Few-shot Classification

Few-shot classification aims to learn a classifier to recognize unseen classes during training with limited labeled examples. While significant progress has been made, the growing complexity of network designs, meta-learning algorithms, and differences in implementation details make a fair comparison difficult. In this paper, we present 1) a consistent comparative analysis of several representative few-shot classification algorithms, with results showing that deeper backbones significantly reduce the performance differences among methods on datasets with limited domain differences, 2) a modified baseline method that surprisingly achieves competitive performance when compared with the state-of-the-art on both the \miniI and the CUB datasets, and 3) a new experimental setting for evaluating the cross-domain generalization ability for few-shot classification algorithms. Our results reveal that reducing intra-class variation is an important factor when the feature backbone is shallow, but not as critical when using deeper backbones. In a realistic cross-domain evaluation setting, we show that a baseline method with a standard fine-tuning practice compares favorably against other state-of-the-art few-shot learning algorithms.

==> figure/fig_domain_difference.tex <==
\begin{minipage}[t]{0.7\textwidth}
\includegraphics[width=\linewidth]{./figure/domain_difference_results.png}
\captionof{figure}{accuracy comparison in different dataset with ResNet18 backbone}
%\caption{accuracy comparison in different dataset with ResNet18 backbone}
\label{fig:domain_difference}
\end{minipage}

==> figure/fig_extra_fine_tune.tex <==
\begin{figure*}[h]
\includegraphics[width=\linewidth]{./figure/fine_tune_results.png}
\caption{Results before and after extra fine-tuning in (a) CUB (b) mini-imagenet (c) cross setting}
\label{fig:finetune}
\end{figure*}

==> figure/fig_motivation.tex <==
\begin{figure}[t]
%\jbox{\textwidth}{0.3\linewidth}
%\caption{Motivation of the method. Main idea.}
%\label{fig:motivation}
\end{figure}

==> figure/fig_nway.tex <==
\begin{figure*}[t]
\includegraphics[width=\linewidth]{./figure/n_way_results.pdf}
\caption{accuracy v.s. n-way classification in training stage for (a) CUB (b) mini-Imagenet dataset. Both are 5-way classification in test stage and are 5-shot.}
\label{fig:nway}
\end{figure*}

==> figure/fig_teaser.tex <==
\begin{center}
%\centering
%\jbox{\textwidth}{0.3\textwidth}
%\captionof{figure}{Teaser figure. Main idea of the paper.}
%\label{fig:teaser}
\end{center}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}



% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> n_way_result_backup.tex <==
\subsection{What if inconsistent n-way classification in training and few-shot stage?}
\input{figure/fig_nway}
A difference between pretrain and meta-learning methods is how many class a classifier would predict during main stage. Pretrain methods retain a classifier for all class all the time, that is, full-way classification. On the other hand, meta-learning methods would sample some class to be predicted at a time to simulate few-shot scenario as mentioned in section~\ref{ssec:meta-learning}. However, [protonet] has mentioned that different number of sampled class, or say, different n-way classification during main stage, would affect the final performance. In the following section, we would deeply investigate its effects. 

Here we test 5-shot setting and gradually change from 5-way to full way classification during main stage, while fix 5-way classification during few-shot stage. We conduct the experiment on Protonet, Matchingnet and Relationnet, while MAML is not included since initialization based method do not support inconsistent n-way classification between main and few-shot stage. A detail here is that more sampled classes indicates larger training batch if query data in each class remain the same. To avoid unreasonable increase in batch size, we reduce query data of each class to keep its production to number of sampled class fixed.

As shown in figure~\ref{fig:nway}, accuracy for both Protonet and Matchingnet grows higher as we increase the number of class to predict, and gradually converges at full-way classification, which means not sample at all. Their performance now much closer to compact-pretrain baseline shown in Table~\ref{CUB_standard}~and~\ref{mini_standard}. 

We argue that compactness is the reason. With a larger n-way classification task in training, data would be enforced to be more compact or otherwise mis-recognized, while there is no need to be so compact in a smaller n. On the other hand, if a method already reach good compactness even with smaller n, its performance would hardly get better. Take Relationnet for example, its initial performance is good but with n-way increasing, the accuracy does not improve and even degrades probably due to the reduced query data in each class. 

However, if compactness is the reason, there is a very intuitive way to improve compactness -- increasing backbone depth. We would discuss it in the next section.


==> table/adapt.tex <==
\begin{table}[t]
\centering
\caption{\tb{Meta-learning methods with further adaptation steps.} Further adaptation improves MatchingNet and MAML, but not for ProtoNet under the scenarios with little domain differences due to inconsistency between the meta-training and meta-testing stages. All statistics are for 5-shot accuracy with ResNet-18 backbone. The notation * indicates that only the new classifiers are updated. The notation $\#$ means the methods are updated for more gradient update steps.}
%\zsolt{So with this update it's still not better than baseline for cross-domain. You don't have the tables for the other cases (resnet-18) so it's hard to tell about those. Perhaps we should discuss in the main body of the section describing whether it does or doesn't catch up to Baseline++}\weiyu{OK!} 
\label{tab:adapt}
\begin{tabular}{ l c | c c c }
\toprule
                             & \small{Adapted}       & \small{CUB}            & \small{\miniI}  & \small{\miniI$\rightarrow$CUB}          \\ \midrule
\small{Baseline}                     & \small{Yes*}          & \small{82.85$\pm$0.55} & \small{74.27$\pm$0.63} & \small{65.57$\pm$0.70} \\  %\midrule
\small{Baseline++}                   & \small{Yes*}          & \small{83.58$\pm$0.54} & \small{75.68$\pm$0.63} & \small{62.04$\pm$0.76} \\ \midrule
\multirow{3}{*}{\small{ProtoNet}}    & \small{No} 	         & \small{87.42$\pm$0.48} & \small{73.68$\pm$0.65} & \small{62.02$\pm$0.70} \\ 
                             & \small{Yes*}          & \small{87.15$\pm$0.50} & \small{72.27$\pm$0.64} & \small{62.68$\pm$0.71} \\ 
                             & \small{Relative Gain} & \small{-0.31$\%$}      & \small{-1.91$\%$}      & \small{1.06$\%$}          \\ \midrule
\multirow{3}{*}{\small{MatchingNet}} & \small{No}            & \small{82.75$\pm$0.58} & \small{68.88$\pm$0.69} & \small{53.07$\pm$0.74} \\  
                             & \small{Yes*}          & \small{84.39$\pm$0.57} & \small{72.92$\pm$0.66} & \small{57.99$\pm$0.77} \\  
                             & \small{Relative Gain} & \small{1.98$\%$}       & \small{5.87$\%$}       & \small{9.27$\%$}          \\ \midrule
\multirow{3}{*}{\small{MAML}}        & \small{No}            & \small{82.70$\pm$0.65} & \small{65.72$\pm$0.77} & \small{51.34$\pm$0.72} \\  
                             & \small{Yes$\#$}       & \small{84.01$\pm$0.58} & \small{70.67$\pm$0.70} & \small{56.03$\pm$0.76} \\ 
                             & \small{Relative Gain} & \small{1.58$\%$}       & \small{7.53$\%$}       & \small{9.14$\%$}          \\ 

\bottomrule
                             
                             
\end{tabular}
\end{table}

==> trashcan/CUB_result.tex <==
% Table - CUB
\begin{table}[t]
\centering
\caption{Few-shot classification on dataset of \textit{Caltech-UCSD Birds 200}.}
\label{CUB_standard}
\begin{tabular}{|l|c|c|c|c|}
\hline
                                       & \multicolumn{2}{c|}{Released statistics} & \multicolumn{2}{c|}{Our Reimplementation} \\ \hline
                                       & 1-shot        & 5-shot & 1-shot               & 5-shot         \\ \hline
Pretrain                               &               &        & 47.12$\pm$0.74       & 64.16$\pm$0.71 \\ \hline
Compact Pretrain                       &               &        & 60.53$\pm$0.83       & 79.34$\pm$0.61 \\ \hline
MatchingNet~\cite{vinyals2016matching} & 49.34         & 59.31  & 54.90$\pm$0.85       & 72.86$\pm$0.70 \\ \hline
ProtoNet~\cite{snell2017prototypical}  &               &        &  40.90$\pm$0.78      & 70.77$\pm$0.69 \\ \hline
ProtoNet(way changing)                    & 45.27         & 34.35  &                      &                \\ \hline
MAML~\cite{finn2017model}              & 38.43         & 59.15  & 53.14$\pm$0.92       & 72.09$\pm$0.76 \\ \hline
Relationnet~\cite{sung2018learning}    &               &        & 56.00$\pm$0.95       & 76.11$\pm$0.69 \\ \hline
\end{tabular}
\end{table}

==> trashcan/mini_imagenet_result.tex <==
% Table - mini_imagenet
\begin{table}[t]
\centering
\caption{Few-shot classification on dataset of \textit{mini-imagenet}.
\jiabin{Avoid using ``hline''. Use toprule, midrule, and bottom rule instead. It will give a better spacing for your table.}
}
\label{mini_standard}
\begin{tabular}{|l|c|c|c|c|}
\toprule
                                       & \multicolumn{2}{c|}{Released statistics} & \multicolumn{2}{c|}{Our Reimplementation} \\ \hline
                                       & 1-shot           & 5-shot          & 1-shot              & 5-shot              \\ \hline
Pretrain                               & 41.08$\pm$0.70   & 51.04$\pm$0.65  & 42.11$\pm$0.71      & 62.53$\pm$0.69      \\ \hline
Compact Pretrain                       &                  &                 & 48.24$\pm$0.75      & 66.43$\pm$0.63      \\ \midrule
Matchingnet~\cite{vinyals2016matching} & 43.56$\pm$0.84   & 55.31$\pm$0.73  & 47.08$\pm$0.79      & 63.48$\pm$0.66      \\ \hline
Protonet~\cite{snell2017prototypical}  &                  &                 & 41.88$\pm$0.79      & 64.24$\pm$0.72      \\ \hline
Protonet(way changing)                   & 49.42$\pm$0.78   & 68.20$\pm$0.66  &                     &                     \\ \hline
MAML~\cite{finn2017model}              & 48.07$\pm$1.75   & 63.15$\pm$0.91  & 46.29$\pm$0.80      & 62.71$\pm$0.71      \\ \hline
Relationnet~\cite{sung2018learning}    & 50.44$\pm$0.82   & 65.32$\pm$0.70  & 47.08$\pm$0.80      & 66.60$\pm$0.69      \\ \bottomrule
\end{tabular}
\end{table}




==> trashcan/overview.tex <==
\section{Overview}
\label{sec:overview}

% Introduce your problem with a toy example

% This figure illustrate the overall process of the algorithm, starting from inputs, processing steps, and outputs. Use forward references the figures with the corresponding equations and sections in the paper.
\input{figure/fig_overview}
